Let's Sample Step by Step: Adaptive-Consistency for Efficient Reasoning and Coding with LLMs

A popular approach for improving the correctness of output from large language models (LLMs) is Self-Consistency - poll the LLM multiple times and output the most frequent solution. Existing Self-Consistency techniques always generate a constant number of samples per question, where a better approach will be to non-uniformly distribute the available budget based on the amount of agreement in the samples generated so far. In response, we introduce Adaptive-Consistency, a cost-efficient, model-agnostic technique that dynamically adjusts the number of samples per question using a lightweight stopping criterion. Our experiments over 17 reasoning and code generation datasets and three LLMs demonstrate that Adaptive-Consistency reduces sample budget by up to 7.9 times with an average accuracy drop of less than 0.1%. Our code and data are available at https://www.sample-step-by-step.info

==> tables/fulltable.tex <==
% \begin{table*}[ht!]
%   \centering
%   \resizebox{0.99\linewidth}{!}{
%     \begin{tabular}{@{}lc|c|cc|cc|cc@{}}
%     \toprule
%       & & \multicolumn{1}{c|} {\textbf{\self}} & \multicolumn{2}{c|}{\textbf{\ours}} & \multicolumn{2}{c}{$\Delta$} \\
%      \cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%      & & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} \\
%      & & & \textbf{{Generations }} & & \textbf{{Generations }} & \\

\begin{table*}[ht!]
  \centering
  \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{}lc|c|cc|cc|cc@{}}
    \toprule
      & & \multicolumn{1}{c|} {\textbf{\self}} & \multicolumn{2}{c|}{\textbf{\ours}} & \multicolumn{2}{c}{$\Delta$} \\
     \cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
     & & \textbf{{Accuracy}} & \textbf{Avg. Gen.} & \textbf{{Accuracy}} &\textbf{Gen. Reduc.} & \textbf{{Acc. Diff. $\uparrow$}} \\
     % & & &  & &  & \\
    \midrule
\addlinespace
\multirow{3}{*}{\textbf{\gsm}} & \vicuna & $\textbf{31.6}$ & $\textbf{26.8}$ & $31.5$ & \boost{$1.4$} & $-0.1$ \\
\addlinespace
 & \codex & $\textbf{81.1}$ & $\textbf{13.8}$ & $81.0$ & \boost{$2.9$} & $-0.1$ \\
 \addlinespace
 & \chatgpt & $\textbf{82.7}$ & $\textbf{9.2}$ & $82.7$ & \boost{$4.3$} & $0.0$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\svamp}} & \vicuna & $\textbf{63.0}$ & $\textbf{18.8}$ & $62.8$ & \boost{$2.1$} & $-0.2$ \\
\addlinespace
 & \codex & $\textbf{85.1}$ & $\textbf{9.5}$ & $85.0$ & \boost{$4.2$} & $-0.1$ \\
\addlinespace
 & \chatgpt & $\textbf{85.1}$ & $\textbf{9.5}$ & $85.0$ & \boost{$4.2$} & $-0.1$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\asdiv}} & \vicuna & $\textbf{64.0}$ & $\textbf{16.5}$ & $\textbf{64.0}$ & \boost{$2.4$} & $0.0$ \\
\addlinespace
 & \codex & $\textbf{83.2}$ & $\textbf{10.0}$ & $83.2$ & \boost{$4.0$} & $0.0$ \\
 \addlinespace
 & \chatgpt & $\textbf{83.0}$ & $\textbf{10.0}$ & $\textbf{83.0}$ & \boost{$4.0$} & $0.0$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\dateunderstanding}} & \vicuna & $59.8$ & $\textbf{17.3}$ & $\textbf{60.2}$ & \boost{$2.3$} & $+0.4$ \\
\addlinespace
 & \codex & $\textbf{80.3}$ & $\textbf{10.7}$ & $79.5$ & \boost{$3.7$} & $-0.8$ \\
\addlinespace
& \chatgpt & $\textbf{77.5}$ & $\textbf{9.1}$ & $77.0$ & \boost{$4.4$} & $-0.5$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\trackingthree}} & \vicuna & $31.8$ & $\textbf{20.3}$ & $\textbf{32.0}$ & \boost{$2.0$} & $+0.2$ \\
\addlinespace
 & \codex & $\textbf{77.2}$ & $\textbf{9.7}$ & $77.1$ & \boost{$4.1$} & $-0.1$ \\
\addlinespace
 & \chatgpt & $85.2$ & $\textbf{6.2}$ & $\textbf{85.6}$ & \boost{$6.4$} & $+0.4$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\logicalthree}} & \vicuna & $51.2$ & $\textbf{18.1}$ & $\textbf{51.4}$ & \boost{$2.2$} & $+0.2$ \\
\addlinespace
 & \codex & $\textbf{89.4}$ & $\textbf{8.5}$ & $\textbf{89.4}$ & \boost{$4.7$} & $0.0$ \\
\addlinespace
 & \chatgpt & $\textbf{86.8}$ & $\textbf{7.5}$ & $\textbf{86.8}$ & \boost{$5.3$} & $0.0$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\strategyqa}} & \vicuna & $65.8$ & $\textbf{16.3}$ & $\textbf{65.8}$ & \boost{$2.5$} & $0.0$ \\
\addlinespace
 & \codex & $\textbf{79.0}$ & $\textbf{11.9}$ & $78.8$ & \boost{$3.4$} & $-0.2$ \\
 \addlinespace
& \chatgpt & $\textbf{68.1}$ & $\textbf{11.8}$ & $67.9$ & \boost{$3.4$} & $-0.2$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\booleanexpressions}} & \vicuna & $\textbf{79.2}$ & $\textbf{16.2}$ & $78.4$ & \boost{$2.5$} & $-0.8$ \\
\addlinespace
 & \codex & $\textbf{94.5}$ & $\textbf{6.6}$ & $\textbf{94.5}$ & \boost{$6.0$} & $0.0$ \\
\addlinespace
 & \chatgpt & $\textbf{93.2}$ & $\textbf{5.0}$ & $92.8$ & \boost{$7.9$} & $-0.4$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\snarks}} & \vicuna & $73.2$ & $\textbf{23.2}$ & $\textbf{73.6}$ & \boost{$1.7$} & $+0.4$ \\
\addlinespace
 & \codex & $\textbf{74.0}$ & $\textbf{12.7}$ & $\textbf{74.0}$ & \boost{$3.1$} & $0.0$ \\
\addlinespace
& \chatgpt & $\textbf{65.7}$ & $\textbf{8.8}$ & $65.2$ & \boost{$4.5$} & $-0.6$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\ruinnames}} & \vicuna & $\textbf{43.6}$ & $\textbf{33.8}$ & $\textbf{43.6}$ & \boost{$1.2$} & $0.0$ \\
\addlinespace
 & \codex & $\textbf{78.0}$ & $\textbf{17.2}$ & $\textbf{78.0}$ & \boost{$2.3$} & $0.0$ \\
\addlinespace
 & \chatgpt & $\textbf{74.8}$ & $\textbf{13.1}$ & $74.0$ & \boost{$3.1$} & $-0.8$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\salienttranslation}} & \vicuna & $\textbf{28.9}$ & $\textbf{28.7}$ & $28.7$ & \boost{$1.2$} & $-0.3$ \\
\addlinespace
 & \codex & $\textbf{64.3}$ & $\textbf{11.8}$ & $\textbf{64.3}$ & \boost{$3.4$} & $0.0$ \\
\addlinespace
  & \chatgpt & $\textbf{56.8}$ & $\textbf{11.1}$ & $\textbf{56.8}$ & \boost{$3.6$} & $0.0$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\disambiguationqa}} & \vicuna & $\textbf{63.7}$ & $\textbf{22.8}$ & $63.5$ & \boost{$1.8$} & $-0.3$ \\
\addlinespace
 & \codex & $74.9$ & $\textbf{13.5}$ & $\textbf{75.1}$ & \boost{$3.0$} & $+0.1$ \\
\addlinespace
 & \chatgpt & $\textbf{62.5}$ & $\textbf{13.9}$ & $\textbf{62.5}$ & \boost{$2.9$} & $0.0$ \\
\addlinespace
\hline
\addlinespace
\multirow{3}{*}{\textbf{\penguins}} & \vicuna & $46.8$ & $\textbf{22.9}$ & $\textbf{47.3}$ & \boost{$1.7$} & $+0.5$ \\
\addlinespace
 & \codex & $83.8$ & $\textbf{11.0}$ & $\textbf{84.0}$ & \boost{$3.6$} & $+0.2$ \\
\addlinespace
& \chatgpt & $\textbf{71.9}$ & $\textbf{14.2}$ & $\textbf{71.9}$ & \boost{$2.8$} & $0.0$ \\
\addlinespace
\hline
    \addlinespace
    \multicolumn{2}{l|}{\textbf{Average}} & \textbf{70.3} & \textbf{14.1} & 70.2 & \textbf{\boost{3.2}} & \textbf{-0.07} \\
    % \multicolumn{2}{l|}{\textbf{Average}} & \textbf{67.2} & \textbf{16.5} & \textbf{67.2} & \textbf{\boost{2.8}} & \textbf{-0.03} \\
    \addlinespace

\bottomrule
  \end{tabular}
  }
\caption{Comparison of \ours with \self on \numdsets diverse reasoning datasets. The table presents the accuracy of \self, the average number of generations (Avg. Gen.) for \ours, and the accuracy of \ours. \self always draws 40 samples. The $\Delta$ columns display the reduction in generations (Gen. Reduc.) and the difference in accuracy (Acc. Diff.) between \self and \ours. The last row shows the average values across all datasets: \ours achieves a 3.2 times reduction in sample budget (\textit{Gen. Reduc.}) compared to \self, while maintaining a minimal average accuracy drop of 0.07\% (\textit{Acc. Diff.}).
% \aman{Fill table, bold consistently, Like with Table 1, remove the @x column and add it as a separate analysis (I'm not 100\% sure, but we should try doing it. Current table is a bit distracting)}
}
 \label{tab:fulltable}
\end{table*}



==> tables/fulltable_noacc.tex <==
% \begin{table*}[h]
%   \centering
%   \resizebox{0.99\linewidth}{!}{
%     \begin{tabular}{@{}lc|cc|c|c|c@{}}
%     \toprule
%      & & \textbf{\self} & \textbf{\ours} & $\Delta$ \\
%      & & \textbf{Average $\downarrow$} & \textbf{Average $\downarrow$} & \textbf{Average $\uparrow$} \\
%      & & \textbf{{Generations }} &  \textbf{{Generations }} & \textbf{{Generations }}  \\
%     \midrule
    % \addlinespace
    % \multirow{2}{*}{\textbf{\gsm}} & \vicuna & $33.8$ & $\textbf{24.7}$ & \boost{$1.4$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{14.0}$ & \boost{$2.9$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\svamp}} & \vicuna & $40.0$ & $\textbf{19.0}$ & \boost{$2.1$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{9.7}$ & \boost{$4.1$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\asdiv}} & \vicuna & $40.0$ & $\textbf{16.7}$ & \boost{$2.4$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{10.2}$ & \boost{$3.9$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\dateunderstanding}} & \vicuna & $40.0$ & $\textbf{17.8}$ & \boost{$2.2$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{11.2}$ & \boost{$3.6$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\trackingthree}} & \vicuna & $6.1$ & $\textbf{3.6}$ & \boost{$1.7$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{10.1}$ & \boost{$4.0$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\logicalthree}} & \vicuna & $6.6$ & $\textbf{2.7}$ & \boost{$2.4$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{8.5}$ & \boost{$4.7$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\strategyqa}} & \vicuna & $40.0$ & $\textbf{16.7}$ & \boost{$2.4$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{12.1}$ & \boost{$3.3$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\booleanexpressions}} & \vicuna & $40.0$ & $\textbf{16.1}$ & \boost{$2.5$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{6.7}$ & \boost{$5.9$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\snarks}} & \vicuna & $40.0$ & $\textbf{22.5}$ & \boost{$1.8$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{12.6}$ & \boost{$3.2$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\ruinnames}} & \vicuna & $40.0$ & $\textbf{34.0}$ & \boost{$1.2$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{17.5}$ & \boost{$2.3$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\salienttranslation}} & \vicuna & $36.8$ & $\textbf{29.1}$ & \boost{$1.3$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{12.3}$ & \boost{$3.3$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\disambiguationqa}} & \vicuna & $40.0$ & $\textbf{23.8}$ & \boost{$1.7$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{14.7}$ & \boost{$2.7$} \\
    % \addlinespace
    % \hline
    % \addlinespace
    % \multirow{2}{*}{\textbf{\penguins}} & \vicuna & $40.0$ & $\textbf{22.4}$ & \boost{$1.8$} \\
    % \addlinespace
    %  & \codex & $40.0$ & $\textbf{11.9}$ & \boost{$3.4$} \\
    % \addlinespace
% \bottomrule
%   \end{tabular}
%   % }
% \caption{Table w/o accuracy. Comparison of \ours with \self  on 13 diverse reasoning datasets. \adaptive{} is more sample efficient than \self{}, with almost negligible drop in accuracy. 
% % \aman{Fill table, bold consistently, Like with Table 1, remove the @x column and add it as a separate analysis (I'm not 100\% sure, but we should try doing it. Current table is a bit distracting)}
% }
%  \label{tab:fulltable_noacc}
% \end{table*}

\begin{table*}[h]
  \centering
  \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{@{}lc|cc|cc|cc|cc@{}}
    \toprule
     & & \textbf{\self} & \textbf{\ours} & $\Delta$ \\
     & & \textbf{Average $\downarrow$} & \textbf{Average $\downarrow$} & \textbf{Average $\uparrow$} \\
     & & \textbf{{Generations }} &  \textbf{{Generations }} & \textbf{{Generations }}  \\
     \midrule
    \addlinespace
    \multirow{2}{*}{\textbf{\gsm}} & \vicuna & $33.8$ & $\textbf{24.7}$ & \boost{$1.4$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{14.0}$ & \boost{$2.9$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\svamp}} & \vicuna & $40.0$ & $\textbf{19.0}$ & \boost{$2.1$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{9.7}$ & \boost{$4.1$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\asdiv}} & \vicuna & $40.0$ & $\textbf{16.7}$ & \boost{$2.4$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{10.2}$ & \boost{$3.9$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\dateunderstanding}} & \vicuna & $40.0$ & $\textbf{17.8}$ & \boost{$2.2$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{11.2}$ & \boost{$3.6$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\trackingthree}} & \vicuna & $6.1$ & $\textbf{3.6}$ & \boost{$1.7$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{10.1}$ & \boost{$4.0$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\logicalthree}} & \vicuna & $6.6$ & $\textbf{2.7}$ & \boost{$2.4$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{8.5}$ & \boost{$4.7$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\strategyqa}} & \vicuna & $40.0$ & $\textbf{16.7}$ & \boost{$2.4$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{12.1}$ & \boost{$3.3$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\booleanexpressions}} & \vicuna & $40.0$ & $\textbf{16.1}$ & \boost{$2.5$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{6.7}$ & \boost{$5.9$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\snarks}} & \vicuna & $40.0$ & $\textbf{22.5}$ & \boost{$1.8$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{12.6}$ & \boost{$3.2$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\ruinnames}} & \vicuna & $40.0$ & $\textbf{34.0}$ & \boost{$1.2$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{17.5}$ & \boost{$2.3$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\salienttranslation}} & \vicuna & $36.8$ & $\textbf{29.1}$ & \boost{$1.3$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{12.3}$ & \boost{$3.3$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\disambiguationqa}} & \vicuna & $40.0$ & $\textbf{23.8}$ & \boost{$1.7$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{14.7}$ & \boost{$2.7$} \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{\penguins}} & \vicuna & $40.0$ & $\textbf{22.4}$ & \boost{$1.8$} \\
    \addlinespace
     & \codex & $40.0$ & $\textbf{11.9}$ & \boost{$3.4$} \\
    \addlinespace
\bottomrule
  \end{tabular}
  }
\caption{Rough Table w/o accuracy. Comparison of \ours with \self  on 13 diverse reasoning datasets. \adaptive{} is more sample efficient than \self{}, with almost negligible drop in accuracy.
}
 \label{tab:fulltable}
\end{table*}



==> tables/logicresults.tex <==
\begin{table*}[h]
  \centering
  \resizebox{0.99\linewidth}{!}{
  % \begin{tabular}{@{}lc|cc|cc|cc|cc@{}}
  %   \toprule
  %    & & \multicolumn{2}{c|}{\textbf{Greedy Decoding}} & \multicolumn{2}{c|} {\textbf{\self{}@40}} & \multicolumn{2}{c|}{\textbf{\adaptive{}}} & \multicolumn{2}{c}{\textbf{\self{}@x}} \\
  %    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
  %    & & \textbf{Average $\downarrow$}& \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} \\
  %    & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & \\
    % \midrule
    \begin{tabular}{@{}lc|cc|cc|cc|cc@{}}
    \toprule
     & & \multicolumn{2}{c|} {\textbf{\self}} & \multicolumn{2}{c|}{\textbf{\ours}} & \multicolumn{2}{c}{$\Delta$} \\
     % & & \multicolumn{2}{c|}{\textbf{Greedy Decoding}} & \multicolumn{2}{c|} {\textbf{\self{}@40}} & \multicolumn{2}{c|}{\textbf{\adaptive{}}} & \multicolumn{2}{c}{\textbf{\self{}@x}} \\
     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
     & & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} \\
     & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & \\
    \midrule
    \addlinespace
    \multirow{2}{*}{\textbf{Date Understanding}} & Vicuna-13B & $40.0$ & $59.9$ & $\textbf{17.5}$ & $\textbf{60.4}$ & $56.3\%$ & $+0.5$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{80.2}$ & $\textbf{10.9}$ & $79.1$ & $72.8\%$ & $-1.1$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{Tracking Three}} & Vicuna-13B & $6.1$ & $\textbf{2.8}$ & $\textbf{3.5}$ & $\textbf{2.8}$ & $42.7\%$ & $0.0$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $78.8$ & $\textbf{9.8}$ & $\textbf{79.2}$ & $75.6\%$ & $+0.4$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{Logical Three}} & Vicuna-13B & $6.6$ & $\textbf{7.6}$ & $\textbf{2.7}$ & $\textbf{7.6}$ & $59.5\%$ & $0.0$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{90.5}$ & $\textbf{8.4}$ & $\textbf{90.5}$ & $79.0\%$ & $0.0$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{StrategyQA}} & Vicuna-13B & $40.0$ & $65.0$ & $\textbf{16.4}$ & $\textbf{65.2}$ & $58.9\%$ & $+0.2$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{79.2}$ & $\textbf{11.7}$ & $78.9$ & $70.9\%$ & $-0.3$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{Boolean Expressions}} & Vicuna-13B & $40.0$ & $\textbf{80.0}$ & $\textbf{15.9}$ & $78.0$ & $60.2\%$ & $-2.0$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{94.8}$ & $\textbf{6.6}$ & $\textbf{94.8}$ & $83.5\%$ & $0.0$ \\
    \addlinespace
\bottomrule
  \end{tabular}
  }
\caption{Results on Logical Reasoning datasets. \adaptive{} outperforms greedy decoding across all datasets and models. \adaptive{} is more sample efficient than \self{}. When both have similar budget, \adaptive{} always improves upon accuracy over \self{}
% \aman{Fill table, bold consistently, Like with Table 1, remove the @x column and add it as a separate analysis (I'm not 100\% sure, but we should try doing it. Current table is a bit distracting)}
}
 \label{tab:logicresults}
\end{table*}


==> tables/miscresults.tex <==
\begin{table*}[htbp]
  \centering
  \resizebox{0.99\linewidth}{!}{
  % \begin{tabular}{@{}lc|cc|cc|cc|cc@{}}
  \begin{tabular}{@{}lc|cc|cc|cc|cc@{}}
    \toprule
     & & \multicolumn{2}{c|} {\textbf{\self}} & \multicolumn{2}{c|}{\textbf{\ours}} & \multicolumn{2}{c}{$\Delta$} \\
     % & & \multicolumn{2}{c|}{\textbf{Greedy Decoding}} & \multicolumn{2}{c|} {\textbf{\self{}@40}} & \multicolumn{2}{c|}{\textbf{\adaptive{}}} & \multicolumn{2}{c}{\textbf{\self{}@x}} \\
     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
     & & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} \\
     & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & \\
    \midrule
    \addlinespace
    \multirow{2}{*}{\textbf{Snarks}} & Vicuna-13B & $40.0$ & $73.6$ & $\textbf{22.4}$ & $\textbf{74.2}$ & $44.0\%$ & $+0.6$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{75.5}$ & $\textbf{12.3}$ & $\textbf{75.5}$ & $69.4\%$ & $0.0$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{Ruin Names}} & Vicuna-13B & $40.0$ & $\textbf{41.2}$ & $\textbf{33.7}$ & $\textbf{41.2}$ & $15.7\%$ & $0.0$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{78.8}$ & $\textbf{17.1}$ & $78.4$ & $57.1\%$ & $-0.4$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{Salient Translation}} & Vicuna-13B & $36.8$ & $\textbf{31.2}$ & $\textbf{28.5}$ & $\textbf{31.2}$ & $22.4\%$ & $0.0$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{64.4}$ & $\textbf{12.0}$ & $64.0$ & $70.1\%$ & $-0.4$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{Disambiguation QA}} & Vicuna-13B & $40.0$ & $64.4$ & $\textbf{23.5}$ & $\textbf{64.8}$ & $41.1\%$ & $+0.4$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $\textbf{74.8}$ & $\textbf{14.3}$ & $\textbf{74.8}$ & $64.4\%$ & $0.0$ \\
    \addlinespace
    \hline
    \addlinespace
    \multirow{2}{*}{\textbf{Penguins}} & Vicuna-13B & $40.0$ & $45.2$ & $\textbf{22.2}$ & $\textbf{45.9}$ & $44.6\%$ & $+0.7$ \\
    \addlinespace
     & Code-Davinci-002 & $40.0$ & $82.9$ & $\textbf{11.3}$ & $\textbf{83.6}$ & $71.6\%$ & $+0.7$ \\
    \addlinespace
\bottomrule
  \end{tabular}
  }
\caption{Results on Miscellaneous datasets. \adaptive{} outperforms greedy decoding across all datasets and models. \adaptive{} is more sample efficient than \self{}. When both have similar budget, \adaptive{} always improves upon accuracy over \self{}}
 \label{tab:miscresults}
\end{table*}


==> tables/results_stop_category.tex <==
% \begin{table*}
% \small
% \centering
% % \setlength\tabcolsep{2.5pt}
%     \begin{tabular}{@{}l|cc|cc|cc|cc|cc|cc@{}}

% \begin{table*}[h]
% \centering
% \tiny
% \setlength\tabcolsep{1.5pt}
%     \begin{tabular}{@{}l|cc|cc|cc|cc|cc|cc@{}}
%     \toprule
%  &  \multicolumn{2}{c|} {\textbf{\random}} & \multicolumn{2}{c|}{\textbf{\majority}} & \multicolumn{2}{c}{\entropy} & \multicolumn{2}{c}{\binomial} &   \multicolumn{2}{c}{\dirichlet} & \multicolumn{2}{c}{\crp} \\
%  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
%  &  \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} \\
%  & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} &\\
% \midrule
% \mathematical & $20.5$ & $66.1$ & $\textbf{14.8}$ & $67.7$ & $16.2$ & $67.9$ & $15.9$ & $67.9$ & $17.0$ & $\textbf{68.0}$& $15.7$ & $67.9$ \\
% \addlinespace
% \commonsense & $20.6$ & $62.1$ & $\textbf{15.5}$ & $64.2$ & $17.9$ & $64.5$ & $18.4$ & $\textbf{64.7}$ & $19.8$ & $64.5$& $\textbf{17.8}$ & $64.6$ \\
% \addlinespace
% \symbolic & $20.7$ & $68.0$ & $\textbf{11.3}$ & $68.9$ & $14.9$ & $69.2$ & $15.0$ & $\textbf{69.3}$ & $17.3$ & $\textbf{69.3}$& $15.1$ & $\textbf{69.3}$ \\
% \addlinespace
% \bottomrule
%   \end{tabular}
% \caption{Add Caption}
%  \label{tab:stoptable_category}
% \end{table*}


==> tables/stopping_comparison.tex <==

\begin{table*}[h]
  \centering
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{@{}lc|c|c|c@{}}
    \toprule
     & \multirow{2}{*}{\textbf{Method}} & {\textbf{Acc@10}} & {\textbf{Acc@15}} & {\textbf{Acc@20}} \\
     % & \multicolumn{2}{c|}{\textbf{\majority}} & \multicolumn{2}{c}{\entropy (\ours)} & \multicolumn{2}{c}{\binomial} &   \multicolumn{2}{c}{\dirichlet} & \multicolumn{2}{c}{\crp} \\
     \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} 
     % \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
     & & \textbf{{Accuracy $\uparrow$}} & \textbf{{Accuracy $\uparrow$}} & \textbf{{Accuracy $\uparrow$}} \\
     % & \textbf{Average $\downarrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} & \textbf{Average $\uparrow$} & \multirow{2}{*}{\textbf{{Accuracy $\uparrow$}}} \\
     % & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} & & \textbf{{Generations }} &\\
    \midrule
\addlinespace

\multirow{6}{*}{\textbf{\gsm}} & \random & $76.1$ & $77.3$ & $78.4$  \\
 & \majority &  $78.4$ & $80.5$ & $81.1$ \\
 & \entropy & $80.1$ & $80.7$ & $81.1$ \\
 & \binomial & $\textbf{80.5}$ & $\textbf{81.0}$ & $\textbf{81.1}$  \\
 & \dirichlet & $80.2$ & $\textbf{81.0}$ & $81.0$  \\
 & \crp & $\textbf{80.5}$ & $\textbf{81.0}$ & $\textbf{81.1}$ \\


\addlinespace
\hline

\multirow{6}{*}{\textbf{\ruinnames}} & \random & $69.7$ & $72.4$ & $78.4$  \\
 & \majority &  $75.2$ & $76.7$ & $77.7$ \\
 & \entropy & $76.4$ & $77.7$ & $\textbf{78.1}$ \\
 & \binomial & $76.4$ & $78.0$ & $\textbf{78.1}$  \\
 & \dirichlet & $76.4$ & $77.9$ & $\textbf{78.1}$  \\
 & \crp & $\textbf{77.1}$ & $\textbf{78.1}$ & $\textbf{78.1}$ \\

 \addlinespace


\bottomrule
  \end{tabular}
  }
\caption{Comparison of various \Stopfunc{}s in \ours. In general, \binomial outperforms \random and \majority by decent margins across all datasets. \binomial has comparable performance to \dirichlet and \crp, but the latter two are much slower. \entropy performs worse to \binomial and also lacks human-interpretable stopping rationale. }

 \label{tab:stoptable_acc}
\end{table*}







